Optimisation in Neurosymbolic Learning Systems

Neurosymbolic AI aims to integrate deep learning with symbolic AI. This integration has many promises, such as decreasing the amount of data required to train a neural network, improving the explainability and interpretability of answers given by models and verifying the correctness of trained systems. We study neurosymbolic learning, where we have both data and background knowledge expressed using symbolic languages. How do we connect the symbolic and neural components to communicate this knowledge? One option is fuzzy reasoning, which studies degrees of truth. For example, being tall is not a binary concept. Instead, probabilistic reasoning studies the probability that something is true or will happen. Our first research question studies how different forms of fuzzy reasoning combine with learning. We find surprising results like a connection to the Raven paradox stating we confirm "ravens are black" when we observe a green apple. In this study, we did not use the background knowledge when we deployed our models after training. In our second research question, we studied how to use background knowledge in deployed models. We developed a new neural network layer based on fuzzy reasoning. Probabilistic reasoning is a natural fit for neural networks, which we usually train to be probabilistic. However, they are expensive to compute and do not scale well to large tasks. In our third research question, we study how to connect probabilistic reasoning with neural networks by sampling to estimate averages, while in the final research question, we study scaling probabilistic neurosymbolic learning to much larger problems than before. Our insight is to train a neural network with synthetic data to predict the result of probabilistic reasoning.

==> appendices/ilr.tex <==
% \section{Dual Problem}
% This section introduces a dual problem to Equation \ref{eq:optim-problem}. This is used extensively in several proofs. 




% \section{Schur-concave t-norms (Proofs)}
% \label{appendix:schur-concave}

% \subsection{Minimal \boost\ function for t-norms}
% \label{appendix:boost-schur-tnorm}

% \begin{theorem}
%     \label{theorem:schur-concave-t-norm}
%     Let $T$ be a Schur-concave t-norm that is strictly cone-increasing at $\revis{T}$ and let $\|\cdot \|$ be a strict norm. Then there is a minimal \boosted\ vector $\minboostv$ for $\truth$ and $\revis{T}$ such that whenever $\truths_i> \truths_j$, then $\minboosts_i - \truths_i\leq \minboosts_j - \truths_j$. 
% \end{theorem}

% \subsection{Closed-form \boost\ function using additive generators}
% \label{appendix:closed-form-additive}
% \begin{proposition}
%     \label{prop:additive-generator}
%     Let $T$ be a Schur-concave t-norm with additive generator $g$ and let $0<\revis{T}\in [T(\truth, \truthc), \revismax{T}]$. 
%     Let $K\in \{0, ..., n-1\}$ denote the number of truth values such that $\minboosts_i=\truths_i$ in Equation \ref{eq:minboost-t-norm-schur-concave}.
%     % Let $N\subseteq \{1, ..., n\}$ be the set of indices $i$ such that the $\minboostv$ from Equation \ref{eq:minboost-t-norm-schur-concave} has $\minboosts_i=\truths_i$. 
%     Then using

%     \begin{equation}
%         \lambda_K = g^ {-1}\left(\frac{1}{n-K}\left(g(\revis{T}) -\sum_{i=1}^K g(\truths^\downarrow_i) - \sum_{i=1}^m g(C_i)\right)\right)
%     \end{equation}

%     in Equation $\ref{eq:minboost-t-norm-schur-concave}$ gives $T(\minboostv, \truthc)=\revis{T}$ if $\minboostv\in [0, 1]^n$. 
% \end{proposition}




% \subsection{$L_1$ minimal \boost\ function for t-norms}
% \label{appendix:boost-schur-t-norm-L1}
% \begin{proposition}
%     Let $\truth\in [0, 1]^n$ and let $T$ be a Schur-concave t-norm that is strictly cone-increasing at $\revis{T}\in [T(\truth, \truthc), \revismax{T}]$. Then there is a value $\lambda\in [0, 1]$ such that the vector $\minboostv$,
%     \begin{equation}
%         \label{eq:minboost-t-norm-schur-concave}
%         \minboosts_i = \begin{cases}
%             \lambda, & \text{if } \truths_i < \lambda, \\
%             \truths_i, & \text{otherwise,}
%         \end{cases}
%     \end{equation}
%     is a minimal \boosted\ vector for $T$ and the $L_1$ norm at $\truth$ and $\revis{T}$.
% \end{proposition}


% \subsection{$L_1$ minimal \boost\ function for t-conorms}
% \label{appendix:schur-concave-t-conorm-l1}
% \begin{proposition}
%     Let $\truth\in [0, 1]^n$ and let $S$ be a Schur-convex t-conorm that is strictly cone-increasing at $\revis{S}\in [S(\truth, \truthc), 1]$. Then there is a value $\lambda\in [0, 1]$ such that the vector $\minboostv$,
%     \begin{equation}
%         \minboosts_i = \begin{cases}
%             \lambda & \text{if } i={\arg\max}_{i\in D}\truths_i, \\
%             \truths_i, & \text{otherwise,}
%         \end{cases}
%     \end{equation}
%     is a minimal \boosted\ vector for $S$ and the $L_1$ norm at $\truth$ and $\revis{S}$.
% \end{proposition}
% \begin{proposition}
%     Let $\truth\in [0, 1]^n$ and let $S$ be a Schur-convex t-conorm that is strictly cone-increasing at $\revis{S}\in [S(\truth, \truthc), 1]$. Then there is a value $\lambda\in [0, 1]$ such that the vector $\minboostv$ with $i\in D$,
%     \begin{equation}
%         \minboosts_i = \begin{cases}
%             \lambda & \text{if } i={\arg\max}_{i\in D}\truths_i, \\
%             \truths_i, & \text{otherwise,}
%         \end{cases}
%     \end{equation}
%     is a minimal \boosted\ vector for $S$ and the $L_1$ norm at $\truth$ and $\revis{S}$.
% \end{proposition}



% \subsection{$L_1$ minimal \boost\ function for residuums}
% \label{appendix:boost-schur-residuum}
% \todo{This doesn't consider constants}
%     \begin{proposition}
%         Let $\truths_1, \truths_2\in [0,1]$ and let $T$ be a strict Schur-concave t-norm with additive generator $g$. Consider its residuum $R(\truths_1, \truths_2)=\sup \{z\vert T(\truths_1, z)\leq \truths_2\}$ that is strictly cone-increasing at $0<\revis{R}\in [R(\truths_1, \truths_2), \revismax{R}]$. Then there is a value $\lambda\in [0, 1]$ such that $\minboostv=[\truths_1, \lambda]^\top$ is a minimal \boosted\ vector for $R$ and the $L_1$ norm at $\truth$ and $\weight$. 
%     \end{proposition}
    


% \section{Product t-norm with $L_2$ norm}
% \label{Appendix:product-l2}
% In this appendix, we consider the \boost\ functions for the product t-norm under the $L_2$-norm. We find that there is no simple closed-form parameterization in terms of $\revis{\varphi}$, but we can find approximations in linear time. These are satisfactory to reliably find the minimal \boost\ function.

% In the following, we wil ignore constants and consider formulas $\bigwedge_{i=1}^n P_i$, and consider the problem in Equation \ref{eq:optim-problem}. We consider the logarithm of the product as its optimum coincides. 

% \begin{equation}
%     \label{eq:optim-problem-prod-p1}
%     \begin{aligned}
%         \textrm{For all } \quad & \truth\in [0,1]^n, \revis{T_P} \in [T_P(\truth), 1] & \\
%         \min_{\boostv} \quad & \sum_{i=1}^n (\boosts_i - \truths_i)^2 & \\
%         \textrm{such that } \quad & \sum_{i=1}^n \log \boosts_i = \log \revis{T_P} \\
%         & \boosts_i-1 \leq 0 
%     \end{aligned}
% \end{equation}
% With Lagrangian $L=\sum_i (\boosts_i - \truths_i)^2 + \lambda(\sum_i \log \boosts_i -\log \revis{T_P})  - \gamma_i(\boosts_i - 1)$, and so
% \begin{align*}
%     \frac{\partial L}{\partial \boosts_i} &= 2(\boosts_i - \truths_i) - \gamma_i +\frac{\lambda}{\boosts_i}=0 \\
%     \lambda &= (\gamma + 2\truths_i - 2\boosts_i) \boosts_i %(\gamma_i-2\boosts_i)(\truths_i + \boosts_i)
% \end{align*}
% Since this holds for all $i$, we find that for all $i$, $j$, $(\gamma + 2\truths_i - 2\boosts_i) \boosts_i= (\gamma + 2\truths_j - 2\boosts_j) \boosts_j=\lambda$. We partition $\{1, ..., n\}$ into sets $I$ and $M$, where $I$ contains all $i$ such that $\boosts_i < 1$, and $M$ those where $\boosts_i=1$. For $i\in I$, by noting that using the complementary slackness condition $\gamma_i=0$, this induces a quadratic equation in $\boosts_i$ with solutions
% \begin{equation}
%     \label{eq:boostv_p2}
%     \boosts_i = \frac{1}{2}(\truths_i \pm \sqrt{\truths_i^2-2\lambda}).
% \end{equation} 
% Since we assume $\boosts_i\geq \truths_i$, we have to take the solution that adds the root of the determinant, that is, $\boosts_i=\frac{1}{2}(\sqrt{\truths_i^2-2\lambda}+\truths_i)$. Furthermore, since we constrain for $i\in I$ that $\boosts_i < 1$, we find that 
% \begin{align*}
%     1 &> \frac{1}{2}(\truths_i + \sqrt{\truths_i^2-2\lambda}) \\
%     2 - \truths_i & > \sqrt{\truths_i^2 - 2\lambda} \\
%     \lambda &> 2\truths_i - 2.
% \end{align*}
% Therefore, given some chosen value of $c$, we require for all $i\in I$ that $\lambda > 2\truths_i - 2$, and so, 
% \begin{equation*}
%     \min_{i\in I} 2\truths_i - 2 >\lambda 
% \end{equation*} 

% Unfortunately, finding the exact value of $\lambda$ such that $T_P(\boostv)=\revis{T_P}$ is a challenge. Filling in $\boosts_i$, we find
% \begin{equation}
%     T_P(\boostv)=\prod_{i=1}^n (\boosts_i)=\prod_{i\in I}\frac{1}{2}(\truths_i+\sqrt{\truths_i^2-2\lambda})=\revis{T_P}.
% \end{equation}
% This is a $2n$-th degree polynomial in $\lambda$, and we were not able to find an obvious, general closed form solution to it. Mathematica \cite{inc.MathematicaVersion12} finds a complicated closed form formula for $n=2$, but cannot find closed form formulas for $n>2$. 

% We also still need to figure out how to partition $i=\{1, ..., n\}$ into $I$ and $M$. Since $\boosts_i$ as computed by Equation \ref{eq:boostv_p2} is a strictly decreasing function in $\lambda$ for all $i\in I$, we have the following unproven proposition. It supports the result given in Theorem \ref{theorem:schur-concave-t-norm} .
% \begin{proposition}
%     For all $\lambda\in[\min_{i=1}^n 2\truths_i-2, 0]$, the function 
%     \begin{equation}
%         \minboost_{T_P}(\truth, \lambda)_i= \begin{cases}
%             \frac{1}{2}(\truths_i + \sqrt{\truths_i^2 - 2\lambda}) & \text{if } 2\truths_i -2 > \lambda, \\
%             1-\truths_i & \text {otherwise.}
%         \end{cases}
%     \end{equation}
%     has the following properties:
%     \begin{enumerate}
%         \item $\minboost_{T_P}(\truth, \lambda)$ is a minimal \boost\ vector for the product t-norm, the $L_2$ norm and $\revis{T_P}=T_P(\minboost_{T_P}(\truth, \lambda))$;
%         \item $\revis{T_P}=T_P(\minboost_{T_P}(\truth, \lambda))$ is a strictly decreasing function in $c$ on $(\min_{i=1}^n 2\truths_i-2, 0]$, and so there is a bijection between $\lambda$ and $\weight \in [T_P(\truth), 1]$ on this interval.
%     \end{enumerate}
% \end{proposition}
% % Do we have a proof for 1 yet?

% The second property is easy to see by noting the derivative of $\minboost_{T_P}(\truth, \lambda)$ is negative on $\lambda \in (\min_{i=1}^n 2\truths_i - 2]$, but for the first we do not have a direct proof as of yet and leave this for future work.

% Although $\minboost_{T_P}(\truth, \lambda)$ is not parameterized in terms of $\revis{T_P}$, it can still be used in practical scenarios where $\lambda$ can  be seen as the negative \say{confidence} in the clause. A practical implementation could learn a weight for the clause between 0 and 1, and then transform it to the domain of $\lambda$ by dividing by $\min_{i=1}^n 2\truths_i - 2$. Alternatively, $\|T_P(\truth+\minboost_{T_P}(\truth, \lambda))-\revis{T_P}\|_2$ can be minimized with respect to $\lambda$ using mathematical optimization methods like gradient descent or Newton's method to find answers in terms of $\revis{T_P}$. 


% \section{Additional experiments}
% \label{appendix:additional-experiments}
% This Appendix presents additional experiments when $\revis{\varphi}$ is not 1. 
% \subsection{Results - \Boosted\ value 0.3}
% Figures \ref{fig:results_91_0.3} and \ref{fig:results_2_0.3} present the results when the \boosted\ value $\revis{\varphi}=0.3$.
% \begin{figure}[H]
%     \includegraphics[width=\linewidth]{results_91_0.3_final.png}
%     \caption{\ale{Comparison of ILR with ADAM on uf20-91 of SATLIB. \Boosted\ value 0.3. The x-axis corresponds to the number of iterations, while the y-axis is the value of $\revis{\varphi}$ in the first row of the grid and the $L_1$ norm in the second row.}}
%     \label{fig:results_91_0.3}
% \end{figure}

% \begin{figure}[H]
%     \includegraphics[width=\linewidth]{results_20_0.3_final.png}
%     \caption{\ale{Comparison of ILR with ADAM on the uf20-91 with 20 clauses. \Boosted\ value 0.3.}}
%     \label{fig:results_2_0.3}
% \end{figure}


% \subsection{Results - \Boosted\ value 0.5}
% Figures \ref{fig:results_91_0.5} and \ref{fig:results_20_0.5} present the results when the \boosted\ value $\revis{\varphi}=0.5$. We note that the satisfaction for ADAM in \luk\ converges above 0.5 in Figure \ref{fig:results_91_0.5}. This means the final truth value is too high, and it has not found a proper solution here. 

% \begin{figure}[H]
%     \includegraphics[width=\linewidth]{results_91_0.5_final.png}
%     \caption{\ale{Comparison of ILR with ADAM on the uf20-91 of SATLIB. \Boosted\ value 0.5.}}
%     \label{fig:results_91_0.5}
% \end{figure}

% \begin{figure}[H]
%     \includegraphics[width=\linewidth]{results_20_0.5_final.png}
%     \caption{\ale{Comparison of ILR with ADAM on the uf20-91 with 20 clauses. \Boosted\ value 0.5.}}
%     \label{fig:results_20_0.5}
% \end{figure}


==> dfl/chapters/3_theory/__latexindent_temp.tex <==
A function $f: \mathbb{R}\rightarrow \mathbb{R}$ is said to be \textit{vanishing} if $f(a)\neq 0$ for all $a\in \mathbb{R}$, i.e. it is nonzero everywhere. \\

==> dfl/chapters/4_method.tex <==
% \section{Model}
% \label{sec:model}
% \begin{align}
%   Q(\lambda,\hat{\lambda})
%   = -\frac{1}{2} P(O \mid \lambda )
%     \sum_s \sum_m \sum_t \gamma_m^{(s)} (t)
%     \Biggl( n\log(2\pi)
%   \mspace{150mu}
%   \notag\\
%      + \log \left| C_m^{(s)} \right|
%      + \left( \mathbf{o}_t - \hat{\mu}_m^{(s)} \right)^T C_m^{(s)-1}
%      \left(\mathbf{o}_t - \hat{\mu}_m^{(s)}\right)
%     \Biggr)
% \end{align}

==> siks-dissertations_8-6.tex <==
% Required packages:


\begin{xltabular}{\linewidth}{@{} l @{\hspace{0.5em}} l @{\hspace{1em}} X @{}}

% \toprule
2016
	&	 01	&	 Syed Saiden Abbas (RUN), Recognition of Shapes by Humans and Machines\\
	&	 02	&	 Michiel Christiaan Meulendijk (UU), Optimizing medication reviews through decision support: prescribing a better pill to swallow\\
	&	 03	&	 Maya Sappelli (RUN), Knowledge Work in Context: User Centered Knowledge Worker Support\\
	&	 04	&	 Laurens Rietveld (VU), Publishing and Consuming Linked Data\\
	&	 05	&	 Evgeny Sherkhonov (UVA), Expanded Acyclic Queries: Containment and an Application in Explaining Missing Answers\\
	&	 06	&	 Michel Wilson (TUD), Robust scheduling in an uncertain environment\\
	&	 07	&	 Jeroen de Man (VU), Measuring and modeling negative emotions for virtual training\\
	&	 08	&	 Matje van de Camp (TiU), A Link to the Past: Constructing Historical Social Networks from Unstructured Data\\
	&	 09	&	 Archana Nottamkandath (VU), Trusting Crowdsourced Information on Cultural Artefacts\\
	&	 10	&	 George Karafotias (VUA), Parameter Control for Evolutionary Algorithms\\
	&	 11	&	 Anne Schuth (UVA), Search Engines that Learn from Their Users\\
	&	 12	&	 Max Knobbout (UU), Logics for Modelling and Verifying Normative Multi-Agent Systems\\
	&	 13	&	 Nana Baah Gyan (VU), The Web, Speech Technologies and Rural Development in West Africa - An ICT4D Approach\\
	&	 14	&	 Ravi Khadka (UU), Revisiting Legacy Software System Modernization\\
	&	 15	&	 Steffen Michels (RUN), Hybrid Probabilistic Logics - Theoretical Aspects, Algorithms and Experiments\\
	&	 16	&	 Guangliang Li (UVA), Socially Intelligent Autonomous Agents that Learn from Human Reward\\
	&	 17	&	 Berend Weel (VU), Towards Embodied Evolution of Robot Organisms\\
	&	 18	&	 Albert Mero\~{n}o Pe\~{n}uela (VU), Refining Statistical Data on the Web\\
	&	 19	&	 Julia Efremova (Tu/e), Mining Social Structures from Genealogical Data\\
	&	 20	&	 Daan Odijk (UVA), Context \& Semantics in News \& Web Search\\
	&	 21	&	 Alejandro Moreno C\'{e}lleri (UT), From Traditional to Interactive Playspaces: Automatic Analysis of Player Behavior in the Interactive Tag Playground\\
	&	 22	&	 Grace Lewis (VU), Software Architecture Strategies for Cyber-Foraging Systems\\
	&	 23	&	 Fei Cai (UVA), Query Auto Completion in Information Retrieval\\
	&	 24	&	 Brend Wanders (UT), Repurposing and Probabilistic Integration of Data; An Iterative and data model independent approach\\
	&	 25	&	 Julia Kiseleva (TU/e), Using Contextual Information to Understand Searching and Browsing Behavior\\
	&	 26	&	 Dilhan Thilakarathne (VU), In or Out of Control: Exploring Computational Models to Study the Role of Human Awareness and Control in Behavioural Choices, with Applications in Aviation and Energy Management Domains\\
	&	 27	&	 Wen Li (TUD), Understanding Geo-spatial Information on Social Media\\
	&	 28	&	 Mingxin Zhang (TUD), Large-scale Agent-based Social Simulation - A study on epidemic prediction and control\\
	&	 29	&	 Nicolas H\"{o}ning (TUD), Peak reduction in decentralised electricity systems - Markets and prices for flexible planning\\
	&	 30	&	 Ruud Mattheij (UvT), The Eyes Have It\\
	&	 31	&	 Mohammad Khelghati (UT), Deep web content monitoring\\
	&	 32	&	 Eelco Vriezekolk (UT), Assessing Telecommunication Service Availability Risks for Crisis Organisations\\
	&	 33	&	 Peter Bloem (UVA), Single Sample Statistics, exercises in learning from just one example\\
	&	 34	&	 Dennis Schunselaar (TUE), Configurable Process Trees: Elicitation, Analysis, and Enactment\\
	&	 35	&	 Zhaochun Ren (UVA), Monitoring Social Media: Summarization, Classification and Recommendation\\
	&	 36	&	 Daphne Karreman (UT), Beyond R2D2: The design of nonverbal interaction behavior optimized for robot-specific morphologies\\
	&	 37	&	 Giovanni Sileno (UvA), Aligning Law and Action - a conceptual and computational inquiry\\
	&	 38	&	 Andrea Minuto (UT), Materials that Matter - Smart Materials meet Art \& Interaction Design\\
	&	 39	&	 Merijn Bruijnes (UT), Believable Suspect Agents; Response and Interpersonal Style Selection for an Artificial Suspect\\
	&	 40	&	 Christian Detweiler (TUD), Accounting for Values in Design\\
	&	 41	&	 Thomas King (TUD), Governing Governance: A Formal Framework for Analysing Institutional Design and Enactment Governance\\
	&	 42	&	 Spyros Martzoukos (UVA), Combinatorial and Compositional Aspects of Bilingual Aligned Corpora\\
	&	 43	&	 Saskia Koldijk (RUN), Context-Aware Support for Stress Self-Management: From Theory to Practice\\
	&	 44	&	 Thibault Sellam (UVA), Automatic Assistants for Database Exploration\\
	&	 45	&	 Bram van de Laar (UT), Experiencing Brain-Computer Interface Control\\
	&	 46	&	 Jorge Gallego Perez (UT), Robots to Make you Happy\\
	&	 47	&	 Christina Weber (UL), Real-time foresight - Preparedness for dynamic innovation networks\\
	&	 48	&	 Tanja Buttler (TUD), Collecting Lessons Learned\\
	&	 49	&	 Gleb Polevoy (TUD), Participation and Interaction in Projects. A Game-Theoretic Analysis\\
	&	 50	&	 Yan Wang (UVT), The Bridge of Dreams: Towards a Method for Operational Performance Alignment in IT-enabled Service Supply Chains\\
	
\midrule
2017
	&	 01	&	 Jan-Jaap Oerlemans (UL), Investigating Cybercrime\\
	&	 02	&	 Sjoerd Timmer (UU), Designing and Understanding Forensic Bayesian Networks using Argumentation\\
	&	 03	&	 Dani\"{e}l Harold Telgen (UU), Grid Manufacturing; A Cyber-Physical Approach with Autonomous Products and Reconfigurable Manufacturing Machines\\
	&	 04	&	 Mrunal Gawade (CWI), Multi-core Parallelism in a Column-store\\
	&	 05	&	 Mahdieh Shadi (UVA), Collaboration Behavior\\
	&	 06	&	 Damir Vandic (EUR), Intelligent Information Systems for Web Product Search\\
	&	 07	&	 Roel Bertens (UU), Insight in Information: from Abstract to Anomaly\\
	&	 08	& 	 Rob Konijn (VU)	, Detecting Interesting Differences:Data Mining in Health Insurance Data using Outlier Detection and Subgroup Discovery\\
	&	 09	&	 Dong Nguyen (UT), Text as Social and Cultural Data: A Computational Perspective on Variation in Text\\
	&	 10	&	 Robby van Delden (UT), (Steering) Interactive Play Behavior\\
	&	 11	&	 Florian Kunneman (RUN), Modelling patterns of time and emotion in Twitter \#anticipointment\\
	&	 12	&	 Sander Leemans (TUE), Robust Process Mining with Guarantees\\
 	&	 13	& 	 Gijs Huisman (UT),  Social Touch Technology - Extending the reach of social touch through haptic technology\\
 	&	 14	&	 Shoshannah Tekofsky (UvT), You Are Who You Play You Are: Modelling Player Traits from Video Game Behavior\\
	&	 15	&	 Peter Berck (RUN),  Memory-Based Text Correction\\
	&	 16	&	 Aleksandr Chuklin (UVA), Understanding and Modeling Users of Modern Search Engines\\
	&	 17	&	 Daniel Dimov (UL), Crowdsourced Online Dispute Resolution\\
	&	 18	&	 Ridho Reinanda (UVA), Entity Associations for Search\\
	&	 19	& 	 Jeroen Vuurens (UT), Proximity of Terms, Texts and Semantic Vectors in Information Retrieval\\
	&	 20	&	 Mohammadbashir Sedighi (TUD), Fostering Engagement in Knowledge Sharing: The Role of Perceived Benefits, Costs and Visibility\\
	&	 21	&	 Jeroen Linssen (UT), Meta Matters in Interactive Storytelling and Serious Gaming (A Play on Worlds)\\
	&	 22	&	 Sara Magliacane (VU), Logics for causal inference under uncertainty\\
	&	 23	&	 David Graus (UVA), Entities of Interest --- Discovery in Digital Traces\\
	&	 24	&	 Chang Wang (TUD), Use of Affordances for Efficient Robot Learning\\
	&	 25	&	 Veruska Zamborlini (VU), Knowledge Representation for Clinical Guidelines, with applications to Multimorbidity Analysis and Literature Search\\
	&	 26	&	 Merel Jung (UT), Socially intelligent robots that understand and respond to human touch\\
	&	 27	&	 Michiel Joosse (UT), Investigating Positioning and Gaze Behaviors of Social Robots: People's Preferences, Perceptions and Behaviors\\
	&	 28	&	 John Klein (VU), Architecture Practices for Complex Contexts\\
	&	 29	&	 Adel Alhuraibi (UvT), From IT-BusinessStrategic Alignment to Performance: A Moderated Mediation Model of Social Innovation, and Enterprise Governance of    IT"\\
	&	 30	&	 Wilma Latuny (UvT), The Power of Facial Expressions\\
	&	 31	&	 Ben Ruijl (UL), Advances in computational methods for QFT calculations\\
	&	 32	& 	 Thaer Samar (RUN), Access to and Retrievability of Content in Web Archives\\
	&	 33	&	 Brigit van Loggem (OU), Towards a Design Rationale for Software Documentation: A Model of Computer-Mediated Activity\\
	&	 34	&	 Maren Scheffel (OU), The Evaluation Framework for Learning Analytics \\
	&	 35	&	 Martine de Vos (VU), Interpreting natural science spreadsheets \\
	&	 36	&	 Yuanhao Guo (UL), Shape Analysis for Phenotype Characterisation from High-throughput Imaging \\
	&	 37	&	 Alejandro Montes Garcia (TUE), WiBAF: A Within Browser Adaptation Framework that Enables Control over Privacy \\
	&	 38	&	 Alex Kayal (TUD), Normative Social Applications \\
	&	 39	&	 Sara Ahmadi (RUN), Exploiting properties of the human auditory system and compressive sensing methods to increase   noise robustness in ASR \\
	&	 40	&	 Altaf Hussain Abro (VUA), Steer your Mind: Computational Exploration of Human Control in Relation to Emotions, Desires and Social Support For applications in human-aware support systems \\
	&	 41	&	 Adnan Manzoor (VUA), Minding a Healthy Lifestyle: An Exploration of Mental Processes and a Smart Environment to Provide Support for a Healthy Lifestyle\\
	&	 42	&	 Elena Sokolova (RUN), Causal discovery from mixed and missing data with applications on ADHD  datasets\\
	&	 43	&	 Maaike de Boer (RUN), Semantic Mapping in Video Retrieval\\
	&	 44	&	 Garm Lucassen (UU), Understanding User Stories - Computational Linguistics in Agile Requirements Engineering\\
	&	 45	&	 Bas Testerink	(UU), Decentralized Runtime Norm Enforcement\\
	&	 46	&	 Jan Schneider	(OU), Sensor-based Learning Support\\
	&	 47	&	 Jie Yang (TUD), Crowd Knowledge Creation Acceleration\\
	&	 48	&	 Angel Suarez (OU), Collaborative inquiry-based learning\\

\midrule
2018
	&	 01	&	 Han van der Aa (VUA), Comparing and Aligning Process Representations \\
	&	 02	&	 Felix Mannhardt (TUE), Multi-perspective Process Mining \\
	&	 03	&	 Steven Bosems (UT), Causal Models For Well-Being: Knowledge Modeling, Model-Driven Development of Context-Aware Applications, and Behavior Prediction\\
	&	 04	&	 Jordan Janeiro (TUD), Flexible Coordination Support for Diagnosis Teams in Data-Centric Engineering Tasks \\
	&	 05	&	 Hugo Huurdeman (UVA), Supporting the Complex Dynamics of the Information Seeking Process \\
	&	 06	&	 Dan Ionita (UT), Model-Driven Information Security Risk Assessment of Socio-Technical Systems \\
	&	 07	&	 Jieting Luo (UU), A formal account of opportunism in multi-agent systems \\
	&	 08	&	 Rick Smetsers (RUN), Advances in Model Learning for Software Systems \\
	&	 09	&	 Xu Xie	(TUD), Data Assimilation in Discrete Event Simulations \\
	&	 10	&	 Julienka Mollee (VUA), Moving forward: supporting physical activity behavior change through intelligent technology \\
	&	 11	&	 Mahdi Sargolzaei (UVA), Enabling Framework for Service-oriented Collaborative Networks \\
	&	 12	&	 Xixi Lu (TUE), Using behavioral context in process mining \\
	&	 13	&	 Seyed Amin Tabatabaei (VUA), Computing a Sustainable Future \\
	&	 14	&	 Bart Joosten (UVT), Detecting Social Signals with Spatiotemporal Gabor Filters \\
	&	 15	&	 Naser Davarzani (UM), Biomarker discovery in heart failure \\
	&	 16	&	 Jaebok Kim (UT), Automatic recognition of engagement and emotion in a group of children \\
	&	 17	&	 Jianpeng Zhang (TUE), On Graph Sample Clustering \\
	&	 18	& 	 Henriette Nakad (UL), De Notaris en Private Rechtspraak \\
	&	 19	&	 Minh Duc Pham (VUA), Emergent relational schemas for RDF \\
	&	 20	&	 Manxia Liu (RUN), Time and Bayesian Networks \\
	&	 21	&	 Aad Slootmaker (OUN), EMERGO: a generic platform for authoring and playing scenario-based serious games \\
	&	 22	&	 Eric Fernandes de Mello Ara\'{u}jo (VUA), Contagious: Modeling the Spread of Behaviours, Perceptions and Emotions in Social Networks \\
	&	 23	&	 Kim Schouten (EUR), Semantics-driven Aspect-Based Sentiment Analysis \\
	&	 24	&	 Jered Vroon (UT), Responsive Social Positioning Behaviour for Semi-Autonomous Telepresence Robots \\
	&	 25	&	 Riste Gligorov (VUA), Serious Games in Audio-Visual Collections \\
	&	 26	& 	 Roelof Anne Jelle de Vries (UT),Theory-Based and Tailor-Made: Motivational Messages for Behavior Change Technology \\
	&	 27	&	 Maikel Leemans (TUE), Hierarchical Process Mining for Scalable Software Analysis \\
	&	 28	&	 Christian Willemse (UT), Social Touch Technologies: How they feel and how they make you feel \\
	&	 29	&	 Yu Gu (UVT), Emotion Recognition from Mandarin Speech \\
	&	 30	&	 Wouter Beek,  The "K" in "semantic web" stands for "knowledge": scaling semantics to the web \\
	
\midrule
2019
	&	 01	&	 Rob van Eijk (UL),Web privacy measurement in real-time bidding systems. A graph-based approach to RTB system classification \\
	&	 02	&	 Emmanuelle Beauxis Aussalet (CWI, UU), Statistics and Visualizations for Assessing Class Size Uncertainty \\
	&	 03	&	 Eduardo Gonzalez Lopez de Murillas (TUE), Process Mining on Databases: Extracting Event Data from Real Life Data Sources \\
	&	 04	&	 Ridho Rahmadi (RUN), Finding stable causal structures from clinical data \\
	& 	 05	&	 Sebastiaan van Zelst (TUE), Process Mining with Streaming Data \\
	&	 06	& 	 Chris Dijkshoorn (VU), Nichesourcing for Improving Access to Linked Cultural Heritage Datasets \\
	&	 07	&	 Soude Fazeli (TUD), Recommender Systems in Social Learning Platforms \\
	& 	 08	&	 Frits de Nijs (TUD), Resource-constrained Multi-agent Markov Decision Processes \\
	&	 09	&	 Fahimeh Alizadeh Moghaddam (UVA), Self-adaptation for energy efficiency in software systems \\
	&	 10	&	 Qing Chuan Ye (EUR), Multi-objective Optimization Methods for Allocation and Prediction \\
	&	 11	&	 Yue Zhao (TUD), Learning Analytics Technology to Understand Learner Behavioral Engagement in MOOCs \\
	&	 12	&	 Jacqueline Heinerman (VU), Better Together \\
	&	 13	&	 Guanliang Chen (TUD), MOOC Analytics: Learner Modeling and Content Generation \\
	&	 14	&	 Daniel Davis (TUD), Large-Scale Learning Analytics: Modeling Learner Behavior \& Improving Learning Outcomes in Massive Open Online Courses \\
	&	 15	&	 Erwin Walraven (TUD), Planning under Uncertainty in Constrained and Partially Observable Environments \\
	&	 16	&	 Guangming Li (TUE), Process Mining based on Object-Centric Behavioral Constraint (OCBC) Models \\
	&	 17	&	 Ali Hurriyetoglu (RUN),Extracting actionable information from microtexts \\
	&	 18	&	 Gerard Wagenaar (UU), Artefacts in Agile Team Communication \\
	&	 19	&	 Vincent Koeman (TUD), Tools for Developing Cognitive Agents \\
	&	 20	&	 Chide Groenouwe (UU), Fostering technically augmented human collective intelligence \\
	&	 21	&	 Cong Liu (TUE), Software Data Analytics: Architectural Model Discovery and Design Pattern Detection \\
	&	 22	&	 Martin van den Berg (VU),Improving IT Decisions with Enterprise Architecture \\
	&	 23	&	 Qin Liu (TUD), Intelligent Control Systems: Learning, Interpreting, Verification\\
	&	 24	&	 Anca Dumitrache (VU),  Truth in Disagreement - Crowdsourcing Labeled Data for Natural Language Processing\\
	&	 25	&	 Emiel van Miltenburg (VU), Pragmatic factors in (automatic) image description \\
	&	 26	&	 Prince Singh (UT), An Integration Platform for Synchromodal Transport \\
	&	 27	&	 Alessandra Antonaci (OUN), The Gamification Design Process applied to (Massive) Open Online Courses\\
	&	 28	&	 Esther Kuindersma (UL), Cleared for take-off: Game-based learning to prepare airline pilots for critical situations \\
	&	 29	&	 Daniel Formolo (VU), Using virtual agents for simulation and training of social skills in safety-critical circumstances \\
	&	 30	&	 Vahid Yazdanpanah (UT), Multiagent Industrial Symbiosis Systems \\
	&	 31	&	 Milan Jelisavcic (VU), Alive and Kicking: Baby Steps in Robotics \\
	&	 32	&	 Chiara Sironi (UM), Monte-Carlo Tree Search for Artificial General Intelligence in Games \\
	&	 33	&	 Anil Yaman (TUE), Evolution of Biologically Inspired Learning in Artificial Neural Networks \\
	&	 34	&	 Negar Ahmadi (TUE), EEG Microstate and Functional Brain Network Features for Classification of Epilepsy and PNES \\
	&	 35	&	 Lisa Facey-Shaw (OUN), Gamification with digital badges in learning programming \\
	&	 36	&	 Kevin Ackermans (OUN), Designing Video-Enhanced Rubrics to Master Complex Skills \\
	&	 37	&	 Jian Fang (TUD), Database Acceleration on FPGAs \\
	&	 38	&	 Akos Kadar (OUN), Learning visually grounded and multilingual representations \\

\midrule
2020
	&	 01	&	 Armon Toubman (UL), Calculated Moves: Generating Air Combat Behaviour \\
	&	 02	&	 Marcos de Paula Bueno (UL), Unraveling Temporal Processes using Probabilistic Graphical Models \\
	&	 03	&	 Mostafa Deghani (UvA), Learning with Imperfect Supervision for Language Understanding \\
	&	 04	&	 Maarten van Gompel (RUN), Context as Linguistic Bridges \\
	&	 05	&	 Yulong Pei (TUE), On local and global structure mining \\
	&	 06	&	 Preethu Rose Anish (UT), Stimulation Architectural Thinking during Requirements Elicitation - An Approach and Tool Support \\
	&	 07	&	 Wim van der Vegt (OUN), Towards a software architecture for reusable game components \\
	&	 08	&	 Ali Mirsoleimani (UL),Structured Parallel Programming for Monte Carlo Tree Search \\
	&	 09	&	 Myriam Traub (UU), Measuring Tool Bias and Improving Data Quality for Digital Humanities Research \\
	&	 10	&	 Alifah Syamsiyah (TUE), In-database Preprocessing for Process Mining \\
	&	 11	&	 Sepideh Mesbah (TUD), Semantic-Enhanced Training Data AugmentationMethods for Long-Tail Entity Recognition Models \\
	&	 12	&	 Ward van Breda (VU), Predictive Modeling in E-Mental Health: Exploring Applicability in Personalised Depression Treatment \\
	&	 13	&	 Marco Virgolin (CWI), Design and Application of Gene-pool Optimal Mixing Evolutionary Algorithms for Genetic Programming \\
	&	 14	&	 Mark Raasveldt (CWI/UL), Integrating Analytics with Relational Databases \\
	&	 15	&	 Konstantinos Georgiadis (OUN),  Smart CAT: Machine Learning for Configurable Assessments in Serious Games \\
	&	 16	&	 Ilona Wilmont (RUN), Cognitive Aspects of Conceptual Modelling \\
	&	 17	&	 Daniele Di Mitri (OUN), The Multimodal Tutor: Adaptive Feedback from Multimodal Experiences \\
  	&	 18	&	 Georgios Methenitis (TUD), Agent Interactions \& Mechanisms in Markets with Uncertainties: Electricity Markets in Renewable Energy Systems \\
	&	 19	&	 Guido van Capelleveen (UT), Industrial Symbiosis Recommender Systems \\
	&	 20	&	 Albert Hankel (VU), Embedding Green ICT Maturity in Organisations \\
	&	 21	&	 Karine da Silva Miras de Araujo (VU), Where is the robot?: Life as it could be \\
	&	 22	&	 Maryam Masoud Khamis (RUN), Understanding complex systems implementation through a modeling approach: the case of e-government in Zanzibar \\
	&	 23	&	 Rianne Conijn (UT), The Keys to Writing: A writing analytics approach to studying writing processes using keystroke logging \\
	&	 24	&	 Lenin da N\'{o}brega Medeiros (VUA/RUN), How are you feeling, human? Towards emotionally supportive chatbots \\
	&	 25	&	 Xin Du (TUE), The Uncertainty in Exceptional Model Mining \\
	&	 26	&	 Krzysztof Leszek Sadowski (UU), GAMBIT: Genetic Algorithm for Model-Based mixed-Integer opTimization \\
	&	 27	&	 Ekaterina Muravyeva (TUD), Personal data and informed consent in an educational context \\
	&	 28	&	 Bibeg Limbu (TUD), Multimodal interaction for deliberate practice: Training complex skills with augmented reality \\
	&	 29	&	 Ioan Gabriel Bucur (RUN), Being Bayesian about Causal Inference \\
	&	 30	&	 Bob Zadok Blok (UL), Creatief, Creatiever, Creatiefst \\
	&	 31	&	 Gongjin Lan (VU), Learning better -- From Baby to Better \\
	&	 32	& 	 Jason Rhuggenaath (TUE), Revenue management in online markets: pricing and online advertising \\
	&	 33	& 	 Rick Gilsing (TUE), Supporting service-dominant business model evaluation in the context of business model innovation \\
	&	 34	&	 Anna Bon (MU), Intervention or Collaboration? Redesigning Information and Communication Technologies for Development \\
	&	 35	&	 Siamak Farshidi (UU), Multi-Criteria Decision-Making in Software Production \\

\midrule
2021
	&	 01	&	 Francisco Xavier Dos Santos Fonseca (TUD),Location-based Games for Social Interaction in Public Space \\
	&	 02	&	 Rijk Mercuur (TUD), Simulating Human Routines: Integrating Social Practice Theory in Agent-Based Models \\
	&	 03	&	 Seyyed Hadi Hashemi (UVA), Modeling Users Interacting with Smart Devices \\
	&	 04	&	 Ioana Jivet (OU), The Dashboard That Loved Me: Designing adaptive learning analytics for self-regulated learning \\
	&	 05	&	 Davide Dell'Anna (UU), Data-Driven Supervision of Autonomous Systems \\
	&	 06	&	 Daniel Davison (UT), "Hey robot, what do you think?" How children learn with a social robot \\
	&	 07	&	 Armel Lefebvre (UU), Research data management for open science \\
	&	 08	&	 Nardie Fanchamps (OU), The Influence of Sense-Reason-Act Programming on Computational Thinking \\
	&	 09	&	 Cristina Zaga (UT), The Design of Robothings. Non-Anthropomorphic and Non-Verbal Robots to Promote Children's Collaboration Through Play \\
	&	 10	&	 Quinten Meertens (UvA), Misclassification Bias in Statistical Learning \\
	&	 11	&	 Anne van Rossum (UL), Nonparametric Bayesian Methods in Robotic Vision \\
	&	 12	&	 Lei Pi (UL), External Knowledge Absorption in Chinese SMEs \\
	&	 13	&	 Bob R. Schadenberg (UT), Robots for Autistic Children: Understanding and Facilitating Predictability for Engagement in Learning \\
	&	 14	&	 Negin Samaeemofrad (UL), Business Incubators: The Impact of Their Support \\
	&	 15	& 	 Onat Ege Adali (TU/e), Transformation of Value Propositions into Resource Re-Configurations through the Business Services Paradigm  \\
	&	 16	&	 Esam A. H. Ghaleb (UM), Bimodal emotion recognition from audio-visual cues \\
	&	 17	&	 Dario Dotti (UM), Human Behavior Understanding  from motion and bodily cues using deep neural networks \\
	&	 18	&	 Remi Wieten (UU), Bridging the Gap Between Informal Sense-Making Tools and Formal Systems - Facilitating the Construction of Bayesian Networks and Argumentation Frameworks \\
	&	 19	&	 Roberto Verdecchia (VU), Architectural Technical Debt: Identification and Management \\
	&	 20	&	 Masoud Mansoury (TU/e), Understanding and Mitigating Multi-Sided Exposure Bias in Recommender Systems \\
	&	 21	&	 Pedro Thiago Timb\'{o} Holanda (CWI), Progressive Indexes \\
	&	 22	&	 Sihang Qiu (TUD), Conversational Crowdsourcing \\
	&	 23	&	 Hugo Manuel Proen\c{c}a (LIACS), Robust rules for prediction and description \\
	&	 24	&	 Kaijie Zhu (TUE), On Efficient Temporal Subgraph Query Processing \\
	&	 25	&	 Eoin Martino Grua (VUA), The Future of E-Health is Mobile: Combining AI and Self-Adaptation to Create Adaptive E-Health Mobile Applications \\
	&	 26	& 	 Benno Kruit (CWI \& VUA), Reading the Grid: Extending Knowledge Bases from Human-readable Tables \\
	&	 27	&	 Jelte van Waterschoot (UT), Personalized and Personal Conversations: Designing Agents Who Want to Connect With You \\
	&	 28	&	 Christoph Selig (UL), Understanding the Heterogeneity of Corporate Entrepreneurship Programs \\

\midrule
2022
	&	 01	&	Judith van Stegeren (UT), Flavor text generation for role-playing video games \\
	&	 02	&	Paulo da Costa (TU/e), Data-driven Prognostics and Logistics Optimisation: A Deep Learning Journey \\
	&	 03	&	Ali el Hassouni (VUA), A Model A Day Keeps The Doctor Away: Reinforcement Learning For Personalized Healthcare \\
	&	 04	&	\"{U}nal Aksu (UU), A Cross-Organizational Process Mining Framework \\
	&	 05	&	Shiwei Liu (TU/e), Sparse Neural Network Training with In-Time Over-Parameterization \\
	&	 06	& 	Reza Refaei Afshar (TU/e), Machine Learning for Ad Publishers in Real Time Bidding \\
	&	 07	&	Sambit Praharaj (OU), Measuring the Unmeasurable? Towards Automatic Co-located Collaboration Analytics \\
	&	 08	&	Maikel L. van Eck (TU/e), Process Mining for Smart Product Design \\
	&	 09	&	Oana Andreea Inel (VUA), Understanding Events: A Diversity-driven Human-Machine Approach \\
	&	 10	&	Felipe Moraes Gomes (TUD), Examining the Effectiveness of Collaborative Search Engines \\
	&	 11	&	Mirjam de Haas (UT), Staying engaged in child-robot interaction, a quantitative approach to studying preschoolers' engagement with robots and tasks during second-language tutoring \\
	&	 12	&	Guanyi Chen (UU),  Computational Generation of Chinese Noun Phrases \\
	&	 13	&	Xander Wilcke (VUA), Machine Learning on Multimodal Knowledge Graphs: Opportunities, Challenges, and Methods for Learning on Real-World Heterogeneous and Spatially-Oriented Knowledge \\
	&	 14	&	Michiel Overeem (UU), Evolution of Low-Code Platforms \\
	&	 15	&	Jelmer Jan Koorn (UU), Work in Process: Unearthing Meaning using Process Mining \\
	&	 16	&	Pieter Gijsbers (TU/e), Systems for AutoML Research \\
	&	 17	&	Laura van der Lubbe (VUA), Empowering vulnerable people with serious games and gamification \\
	&	 18	&	Paris Mavromoustakos Blom (TiU), Player Affect Modelling and Video Game Personalisation \\
	&	 19	&	Bilge Yigit Ozkan (UU), Cybersecurity Maturity Assessment and Standardisation \\
	&	 20	&	Fakhra Jabeen (VUA), Dark Side of the Digital Media - Computational Analysis of Negative Human Behaviors on Social Media \\
	&	 21	&	Seethu Mariyam Christopher (UM), Intelligent Toys for Physical and Cognitive Assessments \\
	&	 22	&	Alexandra Sierra Rativa (TiU), Virtual Character Design and its potential to foster Empathy, Immersion, and Collaboration Skills in Video Games and Virtual Reality Simulations \\
	&	 23	&	Ilir Kola (TUD), Enabling Social Situation Awareness in Support Agents \\
	&	 24	&	Samaneh Heidari (UU), Agents with Social Norms and Values - A framework for agent based social simulations with social norms and personal values \\
	&	 25	&	Anna L.D. Latour (LU), Optimal decision-making under constraints and uncertainty \\
	&	 26	&	Anne Dirkson (LU), Knowledge Discovery from Patient Forums: Gaining novel medical insights from patient experiences \\
	&	 27	&	Christos Athanasiadis (UM), Emotion-aware cross-modal domain adaptation in video sequences \\
	&	 28	&	Onuralp Ulusoy (UU), Privacy in Collaborative Systems \\
	&	 29	&	Jan Kolkmeier (UT), From Head Transform to Mind Transplant: Social Interactions in Mixed Reality \\
	&	 30	&	Dean De Leo (CWI), Analysis of Dynamic Graphs on Sparse Arrays \\
	&	 31	&	Konstantinos Traganos (TU/e), Tackling Complexity in Smart Manufacturing with Advanced Manufacturing Process Management \\
	&	 32	&	Cezara Pastrav (UU), Social simulation for socio-ecological systems \\
	&	 33	&	Brinn Hekkelman (CWI/TUD), Fair Mechanisms for Smart Grid Congestion Management \\
	&	 34	&	Nimat Ullah (VUA), Mind Your Behaviour: Computational Modelling of Emotion \& Desire Regulation for Behaviour Change \\
	&	 35	&	Mike E.U. Ligthart (VUA), Shaping the Child-Robot Relationship: Interaction Design Patterns for a Sustainable Interaction \\

\midrule
2023
	&	 01	&	Bojan Simoski (VUA), Untangling the Puzzle of Digital Health Interventions \\
	&	 02	&	Mariana Rachel Dias da Silva (TiU), Grounded or in flight? What our bodies can tell us about the whereabouts of our thoughts \\
	&	 03	&	Shabnam Najafian (TUD), User Modeling for Privacy-preserving Explanations in Group Recommendations \\
	&	 04	&	Gineke Wiggers (UL), The Relevance of Impact: bibliometric-enhanced legal information retrieval \\
	&	 05	&	Anton Bouter (CWI), Optimal Mixing Evolutionary Algorithms for Large-Scale Real-Valued Optimization, Including Real-World Medical Applications \\
	&	 06	&	António Pereira Barata (UL), Reliable and Fair Machine Learning for Risk Assessment \\
	&	 07	&	Tianjin Huang (TU/e), The Roles of Adversarial Examples on Trustworthiness of Deep Learning \\
	&	 08	&	Lu Yin (TU/e), Knowledge Elicitation using Psychometric Learning \\
	&	 09	&	Xu Wang (VUA), Scientific Dataset Recommendation with Semantic Techniques \\
	&	 10	&	Dennis J.N.J. Soemers (UM), Learning State-Action Features for General Game Playing \\
	&	 11	&	Fawad Taj (VUA), Towards Motivating Machines: Computational Modeling of the Mechanism of Actions for Effective Digital Health Behavior Change Applications \\
	&	 12	&	Tessel Bogaard (VUA), Using Metadata to Understand Search Behavior in Digital Libraries \\
	&	 13	&	Injy Sarhan (UU), Open Information Extraction for Knowledge Representation \\
	&	 14	&	Selma Čaušević (TUD), Energy resilience through self-organization \\
	&	 15	&	Alvaro Henrique Chaim Correia (TU/e), Insights on Learning Tractable Probabilistic Graphical Models \\
	&	 16	&	Peter Blomsma (TiU), Building Embodied Conversational Agents: Observations on human nonverbal behaviour as a resource for the development of artificial characters \\
	&	 17	&	Meike Nauta (UT), Explainable AI and Interpretable Computer Vision – From Oversight to Insight \\
	&	 18	&	Gustavo Penha (TUD), Designing and Diagnosing Models for Conversational Search and Recommendation \\
	&	 19	&	George Aalbers (TiU), Digital Traces of the Mind: Using Smartphones to Capture Signals of Well-Being in Individuals \\
	&	 20	&	Arkadiy Dushatskiy (TUD), Expensive Optimization with Model-Based Evolutionary Algorithms applied to Medical Image Segmentation using Deep Learning \\
	&	 21	&	Gerrit Jan de Bruin (UL), Network Analysis Methods for Smart Inspection in the Transport Domain \\
	&	 22	&	Alireza Shojaifar (UU), Volitional Cybersecurity \\
	&	 23	&	Theo Theunissen (UU), Documentation in Continuous Software Development \\
	&	 24	&	Agathe Balayn (TUD), Practices Towards Hazardous Failure Diagnosis in Machine Learning \\
	&	 25	&	Jurian Baas (UU), Entity Resolution on Historical Knowledge Graphs \\
	&	 26	&	Loek Tonnaer (TU/e), Linearly Symmetry-Based Disentangled Representations and their Out-of-Distribution Behaviour \\
	&	 27	&	Ghada Sokar (TU/e), Learning Continually Under Changing Data Distributions \\
	&	 28	&	Floris den Hengst (VUA), Learning to Behave: Reinforcement Learning in Human Contexts \\

\midrule
2024
	&	 01	&	Daphne Miedema (TU/e), On SQL Learning: Disentangling concepts in data systems education \\
	&	 02	&	Emile van Krieken (VUA), Optimisation in Neurosymbolic Learning Systems \\
	&	 03	&	Feri Wijayanto (RUN), Automated Model Selection for Rasch and Mediation Analysis \\
	&	 04	&	Mike Huisman (Leiden University), Understanding Deep Meta-Learning \\

% \bottomrule
\end{xltabular}


==> siks_description.tex <==
% !TEX root = main.tex
\chapter*{SIKS Dissertatiereeks}
\addcontentsline{toc}{chapter}{SIKS Dissertations}

\begin{multicols}{2}
\scriptsize

\section*{2011}

\setlist[description]{style=nextline}
\begin{description}
	\item [01 Botond Cseke (RUN) ] Variational Algorithms for Bayesian Inference in Latent Gaussian Models
	\item [02 Nick Tinnemeier (UU) ] Organizing Agent Organizations. Syntax and Operational Semantics of an Organization-Oriented Programming Language
	\item [03 Jan Martijn van der Werf (TUE) ] Compositional Design and Verification of Component-Based Information Systems
	\item [04 Hado van Hasselt (UU) ] Insights in Reinforcement Learning; Formal analysis and empirical evaluation of temporal-difference
	\item [05 Bas van der Raadt (VU) ] Enterprise Architecture Coming of Age - Increasing the Performance of an Emerging Discipline.
	\item [06 Yiwen Wang (TUE) ] Semantically-Enhanced Recommendations in Cultural Heritage
	\item [07 Yujia Cao (UT) ] Multimodal Information Presentation for High Load Human Computer Interaction
	\item [08 Nieske Vergunst (UU) ] BDI-based Generation of Robust Task-Oriented Dialogues
	\item [09 Tim de Jong (OU) ] Contextualised Mobile Media for Learning
	\item [10 Bart Bogaert (UvT) ] Cloud Content Contention
	\item [11 Dhaval Vyas (UT) ] Designing for Awareness: An Experience-focused HCI Perspective
	\item [12 Carmen Bratosin (TUE) ] Grid Architecture for Distributed Process Mining
	\item [13 Xiaoyu Mao (UvT) ] Airport under Control. Multiagent Scheduling for Airport Ground Handling
	\item [14 Milan Lovric (EUR) ] Behavioral Finance and Agent-Based Artificial Markets
	\item [15 Marijn Koolen (UvA) ] The Meaning of Structure: the Value of Link Evidence for Information Retrieval
	\item [16 Maarten Schadd (UM) ] Selective Search in Games of Different Complexity
	\item [17 Jiyin He (UVA) ] Exploring Topic Structure: Coherence, Diversity and Relatedness
	\item [18 Mark Ponsen (UM) ] Strategic Decision-Making in complex games
	\item [19 Ellen Rusman (OU) ] The Mind's Eye on Personal Profiles
	\item [20 Qing Gu (VU) ] Guiding service-oriented software engineering - A view-based approach
	\item [21 Linda Terlouw (TUD) ] Modularization and Specification of Service-Oriented Systems
	\item [22 Junte Zhang (UVA) ] System Evaluation of Archival Description and Access
	\item [23 Wouter Weerkamp (UVA) ] Finding People and their Utterances in Social Media
	\item [24 Herwin van Welbergen (UT) ] Behavior Generation for Interpersonal Coordination with Virtual Humans On Specifying, Scheduling and Realizing Multimodal Virtual Human Behavior
	\item [25 Syed Waqar ul Qounain Jaffry (VU) ] Analysis and Validation of Models for Trust Dynamics
	\item [26 Matthijs Aart Pontier (VU) ] Virtual Agents for Human Communication - Emotion Regulation and Involvement-Distance Trade-Offs in Embodied Conversational Agents and Robots
	\item [27 Aniel Bhulai (VU) ] Dynamic website optimization through autonomous management of design patterns
	\item [28 Rianne Kaptein (UVA) ] Effective Focused Retrieval by Exploiting Query Context and Document Structure
	\item [29 Faisal Kamiran (TUE) ] Discrimination-aware Classification
	\item [30 Egon van den Broek (UT) ] Affective Signal Processing (ASP): Unraveling the mystery of emotions
	\item [31 Ludo Waltman (EUR) ] Computational and Game-Theoretic Approaches for Modeling Bounded Rationality
	\item [32 Nees-Jan van Eck (EUR) ] Methodological Advances in Bibliometric Mapping of Science
	\item [33 Tom van der Weide (UU) ] Arguing to Motivate Decisions
	\item [34 Paolo Turrini (UU) ] Strategic Reasoning in Interdependence: Logical and Game-theoretical Investigations
	\item [35 Maaike Harbers (UU) ] Explaining Agent Behavior in Virtual Training
	\item [36 Erik van der Spek (UU) ] Experiments in serious game design: a cognitive approach
	\item [37 Adriana Burlutiu (RUN) ] Machine Learning for Pairwise Data, Applications for Preference Learning and Supervised Network Inference
	\item [38 Nyree Lemmens (UM) ] Bee-inspired Distributed Optimization
	\item [39 Joost Westra (UU) ] Organizing Adaptation using Agents in Serious Games
	\item [40 Viktor Clerc (VU) ] Architectural Knowledge Management in Global Software Development
	\item [41 Luan Ibraimi (UT) ] Cryptographically Enforced Distributed Data Access Control
	\item [42 Michal Sindlar (UU) ] Explaining Behavior through Mental State Attribution
	\item [43 Henk van der Schuur (UU) ] Process Improvement through Software Operation Knowledge
	\item [44 Boris Reuderink (UT) ] Robust Brain-Computer Interfaces
	\item [45 Herman Stehouwer (UvT) ] Statistical Language Models for Alternative Sequence Selection
	\item [46 Beibei Hu (TUD) ] Towards Contextualized Information Delivery: A Rule-based Architecture for the Domain of Mobile Police Work
	\item [47 Azizi Bin Ab Aziz (VU) ] Exploring Computational Models for Intelligent Support of Persons with Depression
	\item [48 Mark Ter Maat (UT) ] Response Selection and Turn-taking for a Sensitive Artificial Listening Agent
	\item [49 Andreea Niculescu (UT) ] Conversational interfaces for task-oriented spoken dialogues: design aspects influencing interaction quality
\end{description}

\section*{2012}

\begin{description}
	\item [02 Muhammad Umair (VU) ] Adaptivity, emotion, and Rationality in Human and Ambient Agent Models
	\item [03 Adam Vanya (VU) ] Supporting Architecture Evolution by Mining Software Repositories
	\item [04 Jurriaan Souer (UU) ] Development of Content Management System-based Web Applications
	\item [05 Marijn Plomp (UU) ] Maturing Interorganisational Information Systems
	\item [06 Wolfgang Reinhardt (OU) ] Awareness Support for Knowledge Workers in Research Networks
	\item [07 Rianne van Lambalgen (VU) ] When the Going Gets Tough: Exploring Agent-based Models of Human Performance under Demanding Conditions
	\item [08 Gerben de Vries (UVA) ] Kernel Methods for Vessel Trajectories
	\item [09 Ricardo Neisse (UT) ] Trust and Privacy Management Support for Context-Aware Service Platforms
	\item [10 David Smits (TUE) ] Towards a Generic Distributed Adaptive Hypermedia Environment
	\item [11 J.C.B. Rantham Prabhakara (TUE) ] Process Mining in the Large: Preprocessing, Discovery, and Diagnostics
	\item [12 Kees van der Sluijs (TUE) ] Model Driven Design and Data Integration in Semantic Web Information Systems
	\item [13 Suleman Shahid (UvT) ] Fun and Face: Exploring non-verbal expressions of emotion during playful interactions
	\item [14 Evgeny Knutov (TUE) ] Generic Adaptation Framework for Unifying Adaptive Web-based Systems
	\item [15 Natalie van der Wal (VU) ] Social Agents. Agent-Based Modelling of Integrated Internal and Social Dynamics of Cognitive and Affective Processes.
	\item [16 Fiemke Both (VU) ] Helping people by understanding them - Ambient Agents supporting task execution and depression treatment
	\item [17 Amal Elgammal (UvT) ] Towards a Comprehensive Framework for Business Process Compliance
	\item [18 Eltjo Poort (VU) ] Improving Solution Architecting Practices
	\item [19 Helen Schonenberg (TUE) ] What's Next? Operational Support for Business Process Execution
	\item [20 Ali Bahramisharif (RUN) ] Covert Visual Spatial Attention, a Robust Paradigm for Brain-Computer Interfacing
	\item [21 Roberto Cornacchia (TUD) ] Querying Sparse Matrices for Information Retrieval
	\item [22 Thijs Vis (UvT) ] Intelligence, politie en veiligheidsdienst: verenigbare grootheden?
	\item [23 Christian Muehl (UT) ] Toward Affective Brain-Computer Interfaces: Exploring the Neurophysiology of Affect during Human Media Interaction
	\item [24 Laurens van der Werff (UT) ] Evaluation of Noisy Transcripts for Spoken Document Retrieval
	\item [25 Silja Eckartz (UT) ] Managing the Business Case Development in Inter-Organizational IT Projects: A Methodology and its Application
	\item [26 Emile de Maat (UVA) ] Making Sense of Legal Text
	\item [27 Hayrettin Gurkok (UT)] Mind the Sheep! User Experience Evaluation \& Brain-Computer Interface Games
	\item [28 Nancy Pascall (UvT) ] Engendering Technology Empowering Women
	\item [29 Almer Tigelaar (UT) ] Peer-to-Peer Information Retrieval
	\item [30 Alina Pommeranz (TUD) ] Designing Human-Centered Systems for Reflective Decision Making
	\item [31 Emily Bagarukayo (RUN) ] A Learning by Construction Approach for Higher Order Cognitive Skills Improvement, Building Capacity and Infrastructure
	\item [32 Wietske Visser (TUD) ] Qualitative multi-criteria preference representation and reasoning
	\item [33 Rory Sie (OUN) ] Coalitions in Cooperation Networks (COCOON)
	\item [34 Pavol Jancura (RUN) ] Evolutionary analysis in PPI networks and applications
	\item [35 Evert Haasdijk (VU) ] Never Too Old To Learn -- On-line Evolution of Controllers in Swarm- and Modular Robotics
	\item [36 Denis Ssebugwawo (RUN) ] Analysis and Evaluation of Collaborative Modeling Processes
	\item [37 Agnes Nakakawa (RUN) ] A Collaboration Process for Enterprise Architecture Creation
	\item [38 Selmar Smit (VU) ] Parameter Tuning and Scientific Testing in Evolutionary Algorithms
	\item [39 Hassan Fatemi (UT) ] Risk-aware design of value and coordination networks
	\item [40 Agus Gunawan (UvT) ] Information Access for SMEs in Indonesia
	\item [41 Sebastian Kelle (OU) ] Game Design Patterns for Learning
	\item [42 Dominique Verpoorten (OU) ] Reflection Amplifiers in self-regulated Learning
	\item [43] Withdrawn
	\item [44 Anna Tordai (VU) ] On Combining Alignment Techniques
	\item [45 Benedikt Kratz (UvT) ] A Model and Language for Business-aware Transactions
	\item [46 Simon Carter (UVA) ] Exploration and Exploitation of Multilingual Data for Statistical Machine Translation
	\item [47 Manos Tsagkias (UVA) ] Mining Social Media: Tracking Content and Predicting Behavior
	\item [48 Jorn Bakker (TUE) ] Handling Abrupt Changes in Evolving Time-series Data
	\item [49 Michael Kaisers (UM) ] Learning against Learning - Evolutionary dynamics of reinforcement learning algorithms in strategic interactions
	\item [50 Steven van Kervel (TUD) ] Ontologogy driven Enterprise Information Systems Engineering
	\item [51 Jeroen de Jong (TUD) ] Heuristics in Dynamic Sceduling; a practical framework with a case study in elevator dispatching
\end{description}

\section*{2013}

\begin{description}
	\item [01 Viorel Milea (EUR) ] News Analytics for Financial Decision Support
	\item [02 Erietta Liarou (CWI) ] MonetDB/DataCell: Leveraging the Column-store Database Technology for Efficient and Scalable Stream Processing
	\item [03 Szymon Klarman (VU) ] Reasoning with Contexts in Description Logics
	\item [04 Chetan Yadati (TUD) ] Coordinating autonomous planning and scheduling
	\item [05 Dulce Pumareja (UT) ] Groupware Requirements Evolutions Patterns
	\item [06 Romulo Goncalves (CWI) ] The Data Cyclotron: Juggling Data and Queries for a Data Warehouse Audience
	\item [07 Giel van Lankveld (UvT) ] Quantifying Individual Player Differences
	\item [08 Robbert-Jan Merk (VU) ] Making enemies: cognitive modeling for opponent agents in fighter pilot simulators
	\item [09 Fabio Gori (RUN) ] Metagenomic Data Analysis: Computational Methods and Applications
	\item [10 Jeewanie Jayasinghe Arachchige (UvT) ] A Unified Modeling Framework for Service Design.
	\item [11 Evangelos Pournaras (TUD) ] Multi-level Reconfigurable Self-organization in Overlay Services
	\item [12 Marian Razavian (VU) ] Knowledge-driven Migration to Services
	\item [13 Mohammad Safiri (UT) ] Service Tailoring: User-centric creation of integrated IT-based homecare services to support independent living of elderly
	\item [14 Jafar Tanha (UVA) ] Ensemble Approaches to Semi-Supervised Learning Learning
	\item [15 Daniel Hennes (UM) ] Multiagent Learning - Dynamic Games and Applications
	\item [16 Eric Kok (UU) ] Exploring the practical benefits of argumentation in multi-agent deliberation
	\item [17 Koen Kok (VU) ] The PowerMatcher: Smart Coordination for the Smart Electricity Grid
	\item [18 Jeroen Janssens (UvT) ] Outlier Selection and One-Class Classification
	\item [19 Renze Steenhuizen (TUD) ] Coordinated Multi-Agent Planning and Scheduling
	\item [20 Katja Hofmann (UvA) ] Fast and Reliable Online Learning to Rank for Information Retrieval
	\item [21 Sander Wubben (UvT) ] Text-to-text generation by monolingual machine translation
	\item [22 Tom Claassen (RUN) ] Causal Discovery and Logic
	\item [23 Patricio de Alencar Silva (UvT) ] Value Activity Monitoring
	\item [24 Haitham Bou Ammar (UM) ] Automated Transfer in Reinforcement Learning
	\item [25 Agnieszka Anna Latoszek-Berendsen (UM) ] Intention-based Decision Support. A new way of representing and implementing clinical guidelines in a Decision Support System
	\item [26 Alireza Zarghami (UT) ] Architectural Support for Dynamic Homecare Service Provisioning
	\item [27 Mohammad Huq (UT) ] Inference-based Framework Managing Data Provenance
	\item [28 Frans van der Sluis (UT) ] When Complexity becomes Interesting: An Inquiry into the Information eXperience
	\item [29 Iwan de Kok (UT) ] Listening Heads
	\item [30 Joyce Nakatumba (TUE) ] Resource-Aware Business Process Management: Analysis and Support
	\item [31 Dinh Khoa Nguyen (UvT) ] Blueprint Model and Language for Engineering Cloud Applications
	\item [32 Kamakshi Rajagopal (OUN) ] Networking For Learning; The role of Networking in a Lifelong Learner's Professional Development
	\item [33 Qi Gao (TUD) ] User Modeling and Personalization in the Microblogging Sphere
	\item [34 Kien Tjin-Kam-Jet (UT) ] Distributed Deep Web Search
	\item [35 Abdallah El Ali (UvA) ] Minimal Mobile Human Computer Interaction
	\item [36 Than Lam Hoang (TUe) ] Pattern Mining in Data Streams
	\item [37 Dirk B\"{o}rner (OUN) ] Ambient Learning Displays
	\item [38 Eelco den Heijer (VU) ] Autonomous Evolutionary Art
	\item [39 Joop de Jong (TUD) ] A Method for Enterprise Ontology based Design of Enterprise Information Systems
	\item [40 Pim Nijssen (UM) ] Monte-Carlo Tree Search for Multi-Player Games
	\item [41 Jochem Liem (UVA) ] Supporting the Conceptual Modelling of Dynamic Systems: A Knowledge Engineering Perspective on Qualitative Reasoning
	\item [42 L\'{e}on Planken (TUD) ] Algorithms for Simple Temporal Reasoning
	\item [43 Marc Bron (UVA) ] Exploration and Contextualization through Interaction and Concepts
\end{description}

\section*{2014}

\begin{description}
	\item [01 Nicola Barile (UU) ] Studies in Learning Monotone Models from Data
	\item [02 Fiona Tuliyano (RUN) ] Combining System Dynamics with a Domain Modeling Method
	\item [03 Sergio Raul Duarte Torres (UT) ] Information Retrieval for Children: Search Behavior and Solutions
	\item [04 Hanna Jochmann-Mannak (UT) ] Websites for children: search strategies and interface design - Three studies on children's search performance and evaluation
	\item [05 Jurriaan van Reijsen (UU) ] Knowledge Perspectives on Advancing Dynamic Capability
	\item [06 Damian Tamburri (VU) ] Supporting Networked Software Development
	\item [07 Arya Adriansyah (TUE) ] Aligning Observed and Modeled Behavior
	\item [08 Samur Araujo (TUD) ] Data Integration over Distributed and Heterogeneous Data Endpoints
	\item [09 Philip Jackson (UvT) ] Toward Human-Level Artificial Intelligence: Representation and Computation of Meaning in Natural Language
	\item [10 Ivan Salvador Razo Zapata (VU) ] Service Value Networks
	\item [11 Janneke van der Zwaan (TUD) ] An Empathic Virtual Buddy for Social Support
	\item [12 Willem van Willigen (VU) ] Look Ma, No Hands: Aspects of Autonomous Vehicle Control
	\item [13 Arlette van Wissen (VU) ] Agent-Based Support for Behavior Change: Models and Applications in Health and Safety Domains
	\item [14 Yangyang Shi (TUD) ] Language Models With Meta-information
	\item [15 Natalya Mogles (VU) ] Agent-Based Analysis and Support of Human Functioning in Complex Socio-Technical Systems: Applications in Safety and Healthcare
	\item [16 Krystyna Milian (VU) ] Supporting trial recruitment and design by automatically interpreting eligibility criteria
	\item [17 Kathrin Dentler (VU) ] Computing healthcare quality indicators automatically: Secondary Use of Patient Data and Semantic Interoperability
	\item [18 Mattijs Ghijsen (UVA) ] Methods and Models for the Design and Study of Dynamic Agent Organizations
	\item [19 Vinicius Ramos (TUE) ] Adaptive Hypermedia Courses: Qualitative and Quantitative Evaluation and Tool Support
	\item [20 Mena Habib (UT) ] Named Entity Extraction and Disambiguation for Informal Text: The Missing Link
	\item [21 Kassidy Clark (TUD) ] Negotiation and Monitoring in Open Environments
	\item [22 Marieke Peeters (UU) ] Personalized Educational Games - Developing agent-supported scenario-based training
	\item [23 Eleftherios Sidirourgos (UvA/CWI) ] Space Efficient Indexes for the Big Data Era
	\item [24 Davide Ceolin (VU) ] Trusting Semi-structured Web Data
	\item [25 Martijn Lappenschaar (RUN) ] New network models for the analysis of disease interaction
	\item [26 Tim Baarslag (TUD) ] What to Bid and When to Stop
	\item [27 Rui Jorge Almeida (EUR) ] Conditional Density Models Integrating Fuzzy and Probabilistic Representations of Uncertainty
	\item [28 Anna Chmielowiec (VU) ] Decentralized k-Clique Matching
	\item [29 Jaap Kabbedijk (UU) ] Variability in Multi-Tenant Enterprise Software
	\item [30 Peter de Cock (UvT) ] Anticipating Criminal Behaviour
	\item [31 Leo van Moergestel (UU) ] Agent Technology in Agile Multiparallel Manufacturing and Product Support
	\item [32 Naser Ayat (UvA) ] On Entity Resolution in Probabilistic Data
	\item [33 Tesfa Tegegne (RUN) ] Service Discovery in eHealth
	\item [34 Christina Manteli (VU) ] The Effect of Governance in Global Software Development: Analyzing Transactive Memory Systems.
	\item [35 Joost van Ooijen (UU) ] Cognitive Agents in Virtual Worlds: A Middleware Design Approach
	\item [36 Joos Buijs (TUE) ] Flexible Evolutionary Algorithms for Mining Structured Process Models
	\item [37 Maral Dadvar (UT) ] Experts and Machines United Against Cyberbullying
	\item [38 Danny Plass-Oude Bos (UT) ] Making brain-computer interfaces better: improving usability through post-processing.
	\item [39 Jasmina Maric (UvT) ] Web Communities, Immigration, and Social Capital
	\item [40 Walter Omona (RUN) ] A Framework for Knowledge Management Using ICT in Higher Education
	\item [41 Frederic Hogenboom (EUR) ] Automated Detection of Financial Events in News Text
	\item [42 Carsten Eijckhof (CWI/TUD) ] Contextual Multidimensional Relevance Models
	\item [43 Kevin Vlaanderen (UU) ] Supporting Process Improvement using Method Increments
	\item [44 Paulien Meesters (UvT) ] Intelligent Blauw. Met als ondertitel: Intelligence-gestuurde politiezorg in gebiedsgebonden eenheden.
	\item [45 Birgit Schmitz (OUN) ] Mobile Games for Learning: A Pattern-Based Approach
	\item [46 Ke Tao (TUD) ] Social Web Data Analytics: Relevance, Redundancy, Diversity
	\item [47 Shangsong Liang (UVA) ] Fusion and Diversification in Information Retrieval
\end{description}

\section*{2015}

\begin{description}
	\item [01 Niels Netten (UvA) ] Machine Learning for Relevance of Information in Crisis Response
	\item [02 Faiza Bukhsh (UvT) ] Smart auditing: Innovative Compliance Checking in Customs Controls
	\item [03 Twan van Laarhoven (RUN) ] Machine learning for network data
	\item [04 Howard Spoelstra (OUN) ] Collaborations in Open Learning Environments
	\item [05 Christoph B\"{o}sch (UT) ] Cryptographically Enforced Search Pattern Hiding
	\item [06 Farideh Heidari (TUD) ] Business Process Quality Computation - Computing Non-Functional Requirements to Improve Business Processes
	\item [07 Maria-Hendrike Peetz (UvA) ] Time-Aware Online Reputation Analysis
	\item [08 Jie Jiang (TUD) ] Organizational Compliance: An agent-based model for designing and evaluating organizational interactions
	\item [09 Randy Klaassen (UT) ] HCI Perspectives on Behavior Change Support Systems
	\item [10 Henry Hermans (OUN) ] OpenU: design of an integrated system to support lifelong learning
	\item [11 Yongming Luo (TUE) ] Designing algorithms for big graph datasets: A study of computing bisimulation and joins
	\item [12 Julie M. Birkholz (VU) ] Modi Operandi of Social Network Dynamics: The Effect of Context on Scientific Collaboration Networks
	\item [13 Giuseppe Procaccianti (VU) ] Energy-Efficient Software
	\item [14 Bart van Straalen (UT) ] A cognitive approach to modeling bad news conversations
	\item [15 Klaas Andries de Graaf (VU) ] Ontology-based Software Architecture Documentation
	\item [16 Changyun Wei (UT) ] Cognitive Coordination for Cooperative Multi-Robot Teamwork
	\item [17 Andr\'{e} van Cleeff (UT) ] Physical and Digital Security Mechanisms: Properties, Combinations and Trade-offs
	\item [18 Holger Pirk (CWI) ] Waste Not, Want Not! - Managing Relational Data in Asymmetric Memories
	\item [19 Bernardo Tabuenca (OUN) ] Ubiquitous Technology for Lifelong Learners
	\item [20 Lois Vanh\'{e}e (UU) ] Using Culture and Values to Support Flexible Coordination
	\item [21 Sibren Fetter (OUN) ] Using Peer-Support to Expand and Stabilize Online Learning
	\item [22 Zhemin Zhu (UT) ] Co-occurrence Rate Networks
	\item [23 Luit Gazendam (VU) ] Cataloguer Support in Cultural Heritage
	\item [24 Richard Berendsen (UVA) ] Finding People, Papers, and Posts: Vertical Search Algorithms and Evaluation
	\item [25 Steven Woudenberg (UU) ] Bayesian Tools for Early Disease Detection
	\item [26 Alexander Hogenboom (EUR) ] Sentiment Analysis of Text Guided by Semantics and Structure
	\item [27 S\'{a}ndor H\'{e}man (CWI) ] Updating compressed colomn stores
	\item [28 Janet Bagorogoza (TiU) ] Knowledge Management and High Performance; The Uganda Financial Institutions Model for HPO
	\item [29 Hendrik Baier (UM) ] Monte-Carlo Tree Search Enhancements for One-Player and Two-Player Domains
	\item [30 Kiavash Bahreini (OU) ] Real-time Multimodal Emotion Recognition in E-Learning
	\item [31 Yakup Ko\c{c} (TUD) ] On the robustness of Power Grids
	\item [32 Jerome Gard (UL) ] Corporate Venture Management in SMEs
	\item [33 Frederik Schadd (TUD) ] Ontology Mapping with Auxiliary Resources
	\item [34 Victor de Graaf (UT) ] Gesocial Recommender Systems
	\item [35 Jungxao Xu (TUD) ] Affective Body Language of Humanoid Robots: Perception and Effects in Human Robot Interaction
\end{description}

\section*{2016}

\begin{description}
	\item [01 Syed Saiden Abbas (RUN) ] Recognition of Shapes by Humans and Machines
	\item [02 Michiel Christiaan Meulendijk (UU) ] Optimizing medication reviews through decision support: prescribing a better pill to swallow
	\item [03 Maya Sappelli (RUN) ] Knowledge Work in Context: User Centered Knowledge Worker Support
	\item [04 Laurens Rietveld (VU) ] Publishing and Consuming Linked Data
	\item [05 Evgeny Sherkhonov (UVA) ] Expanded Acyclic Queries: Containment and an Application in Explaining Missing Answers
	\item [06 Michel Wilson (TUD) ] Robust scheduling in an uncertain environment
	\item [07 Jeroen de Man (VU) ] Measuring and modeling negative emotions for virtual training
	\item [08 Matje van de Camp (TiU) ] A Link to the Past: Constructing Historical Social Networks from Unstructured Data
	\item [09 Archana Nottamkandath (VU) ] Trusting Crowdsourced Information on Cultural Artefacts
	\item [10 George Karafotias (VUA) ] Parameter Control for Evolutionary Algorithms
	\item [11 Anne Schuth (UVA) ] Search Engines that Learn from Their Users
	\item [12 Max Knobbout (UU) ] Logics for Modelling and Verifying Normative Multi-Agent Systems
	\item [13 Nana Baah Gyan (VU) ] The Web, Speech Technologies and Rural Development in West Africa - An ICT4D Approach
	\item [14 Ravi Khadka (UU) ] Revisiting Legacy Software System Modernization
	\item [15 Steffen Michels (RUN) ] Hybrid Probabilistic Logics - Theoretical Aspects, Algorithms and Experiments
	\item [16 Guangliang Li (UVA) ] Socially Intelligent Autonomous Agents that Learn from Human Reward
	\item [17 Berend Weel (VU) ] Towards Embodied Evolution of Robot Organisms
	\item [18 Albert Mero\~{n}o Pe\~{n}uela (VU) ] Refining Statistical Data on the Web
	\item [19 Julia Efremova (Tu/e) ] Mining Social Structures from Genealogical Data
	\item [20 Daan Odijk (UVA)] Context \& Semantics in News \& Web Search
	\item [21 Alejandro Moreno C\'{e}lleri (UT) ] From Traditional to Interactive Playspaces: Automatic Analysis of Player Behavior in the Interactive Tag Playground
	\item [22 Grace Lewis (VU) ] Software Architecture Strategies for Cyber-Foraging Systems
	\item [23 Fei Cai (UVA) ] Query Auto Completion in Information Retrieval
	\item [24 Brend Wanders (UT) ] Repurposing and Probabilistic Integration of Data; An Iterative and data model independent approach
	\item [25 Julia Kiseleva (TU/e) ] Using Contextual Information to Understand Searching and Browsing Behavior
	\item [26 Dilhan Thilakarathne (VU) ] In or Out of Control: Exploring Computational Models to Study the Role of Human Awareness and Control in Behavioural Choices, with Applications in Aviation and Energy Management Domains
	\item [27 Wen Li (TUD) ] Understanding Geo-spatial Information on Social Media
	\item [28 Mingxin Zhang (TUD) ] Large-scale Agent-based Social Simulation - A study on epidemic prediction and control
	\item [29 Nicolas H\"{o}ning (TUD) ] Peak reduction in decentralised electricity systems - Markets and prices for flexible planning
	\item [30 Ruud Mattheij (UvT) ] The Eyes Have It
	\item [31 Mohammad Khelghati (UT) ] Deep web content monitoring
	\item [32 Eelco Vriezekolk (UT) ] Assessing Telecommunication Service Availability Risks for Crisis Organisations
	\item [33 Peter Bloem (UVA) ] Single Sample Statistics, exercises in learning from just one example
	\item [34 Dennis Schunselaar (TUE) ] Configurable Process Trees: Elicitation, Analysis, and Enactment
	\item [35 Zhaochun Ren (UVA) ] Monitoring Social Media: Summarization, Classification and Recommendation
	\item [36 Daphne Karreman (UT) ] Beyond R2D2: The design of nonverbal interaction behavior optimized for robot-specific morphologies
	\item [37 Giovanni Sileno (UvA) ] Aligning Law and Action - a conceptual and computational inquiry
	\item [38 Andrea Minuto (UT)] Materials that Matter - Smart Materials meet Art \& Interaction Design
	\item [39 Merijn Bruijnes (UT) ] Believable Suspect Agents; Response and Interpersonal Style Selection for an Artificial Suspect
	\item [40 Christian Detweiler (TUD) ] Accounting for Values in Design
	\item [41 Thomas King (TUD) ] Governing Governance: A Formal Framework for Analysing Institutional Design and Enactment Governance
	\item [42 Spyros Martzoukos (UVA) ] Combinatorial and Compositional Aspects of Bilingual Aligned Corpora
	\item [43 Saskia Koldijk (RUN) ] Context-Aware Support for Stress Self-Management: From Theory to Practice
	\item [44 Thibault Sellam (UVA) ] Automatic Assistants for Database Exploration
	\item [45 Bram van de Laar (UT) ] Experiencing Brain-Computer Interface Control
	\item [46 Jorge Gallego Perez (UT) ] Robots to Make you Happy
	\item [47 Christina Weber (UL) ] Real-time foresight - Preparedness for dynamic innovation networks
	\item [48 Tanja Buttler (TUD) ] Collecting Lessons Learned
	\item [49 Gleb Polevoy (TUD) ] Participation and Interaction in Projects. A Game-Theoretic Analysis
	\item [50 Yan Wang (UVT) ] The Bridge of Dreams: Towards a Method for Operational Performance Alignment in IT-enabled Service Supply Chains
\end{description}

\section*{2017}

\begin{description}
	\item [01 Jan-Jaap Oerlemans (UL) ] Investigating Cybercrime
	\item [02 Sjoerd Timmer (UU) ] Designing and Understanding Forensic Bayesian Networks using Argumentation
	\item [03 Dani\"{e}l Harold Telgen (UU) ] Grid Manufacturing; A Cyber-Physical Approach with Autonomous Products and Reconfigurable Manufacturing Machines
	\item [04 Mrunal Gawade (CWI) ] Multi-core Parallelism in a Column-store
	\item [05 Mahdieh Shadi (UVA) ] Collaboration Behavior
	\item [06 Damir Vandic (EUR) ] Intelligent Information Systems for Web Product Search
	\item [07 Roel Bertens (UU) ] Insight in Information: from Abstract to Anomaly
	\item [08 Rob Konijn (VU)	] Detecting Interesting Differences:Data Mining in Health Insurance Data using Outlier Detection and Subgroup Discovery
	\item [09 Dong Nguyen (UT) ] Text as Social and Cultural Data: A Computational Perspective on Variation in Text
	\item [10 Robby van Delden (UT) ] (Steering) Interactive Play Behavior
	\item [11 Florian Kunneman (RUN) ] Modelling patterns of time and emotion in Twitter \#anticipointment
	\item [12 Sander Leemans (TUE) ] Robust Process Mining with Guarantees
	\item [13 Gijs Huisman (UT) ] Social Touch Technology - Extending the reach of social touch through haptic technology
	\item [14 Shoshannah Tekofsky (UvT) ] You Are Who You Play You Are: Modelling Player Traits from Video Game Behavior
	\item [15 Peter Berck (RUN) ] Memory-Based Text Correction
	\item [16 Aleksandr Chuklin (UVA) ] Understanding and Modeling Users of Modern Search Engines
	\item [17 Daniel Dimov (UL) ] Crowdsourced Online Dispute Resolution
	\item [18 Ridho Reinanda (UVA) ] Entity Associations for Search
	\item [19 Jeroen Vuurens (UT) ] Proximity of Terms, Texts and Semantic Vectors in Information Retrieval
	\item [20 Mohammadbashir Sedighi (TUD) ] Fostering Engagement in Knowledge Sharing: The Role of Perceived Benefits, Costs and Visibility
	\item [21 Jeroen Linssen (UT) ] Meta Matters in Interactive Storytelling and Serious Gaming (A Play on Worlds)
	\item [22 Sara Magliacane (VU) ] Logics for causal inference under uncertainty
	\item [23 David Graus (UVA) ] Entities of Interest --- Discovery in Digital Traces
	\item [24 Chang Wang (TUD) ] Use of Affordances for Efficient Robot Learning
	\item [25 Veruska Zamborlini (VU) ] Knowledge Representation for Clinical Guidelines, with applications to Multimorbidity Analysis and Literature Search
	\item [26 Merel Jung (UT) ] Socially intelligent robots that understand and respond to human touch
	\item [27 Michiel Joosse (UT) ] Investigating Positioning and Gaze Behaviors of Social Robots: People's Preferences, Perceptions and Behaviors
	\item [28 John Klein (VU) ] Architecture Practices for Complex Contexts
	\item [29 Adel Alhuraibi (UvT) ] From IT-BusinessStrategic Alignment to Performance: A Moderated Mediation Model of Social Innovation, and Enterprise Governance of    IT"
	\item [30 Wilma Latuny (UvT) ] The Power of Facial Expressions
	\item [31 Ben Ruijl (UL) ] Advances in computational methods for QFT calculations
	\item [32 Thaer Samar (RUN) ] Access to and Retrievability of Content in Web Archives
	\item [33 Brigit van Loggem (OU) ] Towards a Design Rationale for Software Documentation: A Model of Computer-Mediated Activity
	\item [34 Maren Scheffel (OU) ] The Evaluation Framework for Learning Analytics
	\item [35 Martine de Vos (VU) ] Interpreting natural science spreadsheets
	\item [36 Yuanhao Guo (UL) ] Shape Analysis for Phenotype Characterisation from High-throughput Imaging
	\item [37 Alejandro Montes Garcia (TUE) ] WiBAF: A Within Browser Adaptation Framework that Enables Control over Privacy
	\item [38 Alex Kayal (TUD) ] Normative Social Applications
	\item [39 Sara Ahmadi (RUN) ] Exploiting properties of the human auditory system and compressive sensing methods to increase   noise robustness in ASR
	\item [40 Altaf Hussain Abro (VUA) ] Steer your Mind: Computational Exploration of Human Control in Relation to Emotions, Desires and Social Support For applications in human-aware support systems
	\item [41 Adnan Manzoor (VUA) ] Minding a Healthy Lifestyle: An Exploration of Mental Processes and a Smart Environment to Provide Support for a Healthy Lifestyle
	\item [42 Elena Sokolova (RUN) ] Causal discovery from mixed and missing data with applications on ADHD  datasets
	\item [43 Maaike de Boer (RUN) ] Semantic Mapping in Video Retrieval
	\item [44 Garm Lucassen (UU) ] Understanding User Stories - Computational Linguistics in Agile Requirements Engineering
	\item [45 Bas Testerink	(UU) ] Decentralized Runtime Norm Enforcement
	\item [46 Jan Schneider	(OU) ] Sensor-based Learning Support
	\item [47 Jie Yang (TUD) ] Crowd Knowledge Creation Acceleration
	\item [48 Angel Suarez (OU) ] Collaborative inquiry-based learning
\end{description}

\section*{2018}

\begin{description}
	\item [01 Han van der Aa (VUA) ] Comparing and Aligning Process Representations
	\item [02 Felix Mannhardt (TUE) ] Multi-perspective Process Mining
	\item [03 Steven Bosems (UT) ] Causal Models For Well-Being: Knowledge Modeling, Model-Driven Development of Context-Aware Applications, and Behavior Prediction
	\item [04 Jordan Janeiro (TUD) ] Flexible Coordination Support for Diagnosis Teams in Data-Centric Engineering Tasks
	\item [05 Hugo Huurdeman (UVA) ] Supporting the Complex Dynamics of the Information Seeking Process
	\item [06 Dan Ionita (UT) ] Model-Driven Information Security Risk Assessment of Socio-Technical Systems
	\item [07 Jieting Luo (UU) ] A formal account of opportunism in multi-agent systems
	\item [08 Rick Smetsers (RUN) ] Advances in Model Learning for Software Systems
	\item [09 Xu Xie	(TUD) ] Data Assimilation in Discrete Event Simulations
	\item [10 Julienka Mollee (VUA) ] Moving forward: supporting physical activity behavior change through intelligent technology
	\item [11 Mahdi Sargolzaei (UVA) ] Enabling Framework for Service-oriented Collaborative Networks
	\item [12 Xixi Lu (TUE) ] Using behavioral context in process mining
	\item [13 Seyed Amin Tabatabaei (VUA) ] Computing a Sustainable Future
	\item [14 Bart Joosten (UVT) ] Detecting Social Signals with Spatiotemporal Gabor Filters
	\item [15 Naser Davarzani (UM) ] Biomarker discovery in heart failure
	\item [16 Jaebok Kim (UT) ] Automatic recognition of engagement and emotion in a group of children
	\item [17 Jianpeng Zhang (TUE) ] On Graph Sample Clustering
	\item [18 Henriette Nakad (UL) ] De Notaris en Private Rechtspraak
	\item [19 Minh Duc Pham (VUA) ] Emergent relational schemas for RDF
	\item [20 Manxia Liu (RUN) ] Time and Bayesian Networks
	\item [21 Aad Slootmaker (OUN) ] EMERGO: a generic platform for authoring and playing scenario-based serious games
	\item [22 Eric Fernandes de Mello Araujo (VUA) ] Contagious: Modeling the Spread of Behaviours, Perceptions and Emotions in Social Networks
	\item [23 Kim Schouten (EUR) ] Semantics-driven Aspect-Based Sentiment Analysis
	\item [24 Jered Vroon (UT) ] Responsive Social Positioning Behaviour for Semi-Autonomous Telepresence Robots
	\item [25 Riste Gligorov (VUA) ] Serious Games in Audio-Visual Collections
	\item [26 Roelof Anne Jelle de Vries (UT) ] Theory-Based and Tailor-Made: Motivational Messages for Behavior Change Technology
	\item [27 Maikel Leemans (TUE) ] Hierarchical Process Mining for Scalable Software Analysis
	\item [28 Christian Willemse (UT) ] Social Touch Technologies: How they feel and how they make you feel
	\item [29 Yu Gu (UVT) ] Emotion Recognition from Mandarin Speech
	\item [30 Wouter Beek ] The "K" in "semantic web" stands for "knowledge": scaling semantics to the web
\end{description}

\section*{2019}

\begin{description}
	\item [01 Rob van Eijk (UL) ] Web privacy measurement in real-time bidding systems. A graph-based approach to RTB system classification
	\item [02 Emmanuelle Beauxis Aussalet (CWI, UU) ] Statistics and Visualizations for Assessing Class Size Uncertainty
	\item [03 Eduardo Gonzalez Lopez de Murillas (TUE) ] Process Mining on Databases: Extracting Event Data from Real Life Data Sources
	\item [04 Ridho Rahmadi (RUN) ] Finding stable causal structures from clinical data
	\item [05 Sebastiaan van Zelst (TUE) ] Process Mining with Streaming Data
	\item [06 Chris Dijkshoorn (VU) ] Nichesourcing for Improving Access to Linked Cultural Heritage Datasets
	\item [07 Soude Fazeli (TUD) ] Recommender Systems in Social Learning Platforms
	\item [08 Frits de Nijs (TUD) ] Resource-constrained Multi-agent Markov Decision Processes
	\item [09 Fahimeh Alizadeh Moghaddam (UVA) ] Self-adaptation for energy efficiency in software systems
	\item [10 Qing Chuan Ye (EUR) ] Multi-objective Optimization Methods for Allocation and Prediction
	\item [11 Yue Zhao (TUD) ] Learning Analytics Technology to Understand Learner Behavioral Engagement in MOOCs
	\item [12 Jacqueline Heinerman (VU) ] Better Together
	\item [13 Guanliang Chen (TUD) ] MOOC Analytics: Learner Modeling and Content Generation
	\item [14 Daniel Davis (TUD) ] Large-Scale Learning Analytics: Modeling Learner Behavior \& Improving Learning Outcomes in Massive Open Online Courses
	\item [15 Erwin Walraven (TUD) ] Planning under Uncertainty in Constrained and Partially Observable Environments
	\item [16 Guangming Li (TUE) ] Process Mining based on Object-Centric Behavioral Constraint (OCBC) Models
	\item [17 Ali Hurriyetoglu (RUN) ] Extracting actionable information from microtexts
	\item [18 Gerard Wagenaar (UU) ] Artefacts in Agile Team Communication
	\item [19 Vincent Koeman (TUD) ] Tools for Developing Cognitive Agents
	\item [20 Chide Groenouwe (UU) ] Fostering technically augmented human collective intelligence
	\item [21 Cong Liu (TUE) ] Software Data Analytics: Architectural Model Discovery and Design Pattern Detection
	\item [22 Martin van den Berg (VU) ] Improving IT Decisions with Enterprise Architecture
	\item [23 Qin Liu (TUD) ] Intelligent Control Systems: Learning, Interpreting, Verification
	\item [24 Anca Dumitrache (VU) ] Truth in Disagreement - Crowdsourcing Labeled Data for Natural Language Processing
	\item [25 Emiel van Miltenburg (VU) ] Pragmatic factors in (automatic) image description
	\item [26 Prince Singh (UT) ] An Integration Platform for Synchromodal Transport
	\item [27 Alessandra Antonaci (OUN) ] The Gamification Design Process applied to (Massive) Open Online Courses
	\item [28 Esther Kuindersma (UL) ] Cleared for take-off: Game-based learning to prepare airline pilots for critical situations
	\item [29 Daniel Formolo (VU) ] Using virtual agents for simulation and training of social skills in safety-critical circumstances
	\item [30 Vahid Yazdanpanah (UT) ] Multiagent Industrial Symbiosis Systems
	\item [31 Milan Jelisavcic (VU) ] Alive and Kicking: Baby Steps in Robotics
	\item [32 Chiara Sironi (UM) ] Monte-Carlo Tree Search for Artificial General Intelligence in Games
	\item [33 Anil Yaman (TUE) ] Evolution of Biologically Inspired Learning in Artificial Neural Networks
	\item [34 Negar Ahmadi (TUE) ] EEG Microstate and Functional Brain Network Features for Classification of Epilepsy and PNES
	\item [35 Lisa Facey-Shaw (OUN) ] Gamification with digital badges in learning programming
	\item [36 Kevin Ackermans (OUN) ] Designing Video-Enhanced Rubrics to Master Complex Skills
	\item [37 Jian Fang (TUD) ] Database Acceleration on FPGAs
	\item [38 Akos Kadar (OUN) ] Learning visually grounded and multilingual representations
\end{description}

\section*{2020}

\begin{description}
	\item [01 Armon Toubman (UL) ] Calculated Moves: Generating Air Combat Behaviour
	\item [02 Marcos de Paula Bueno (UL) ] Unraveling Temporal Processes using Probabilistic Graphical Models
	\item [03 Mostafa Deghani (UvA) ] Learning with Imperfect Supervision for Language Understanding
	\item [04 Maarten van Gompel (RUN) ] Context as Linguistic Bridges
	\item [05 Yulong Pei (TUE) ] On local and global structure mining
	\item [06 Preethu Rose Anish (UT) ] Stimulation Architectural Thinking during Requirements Elicitation - An Approach and Tool Support
	\item [07 Wim van der Vegt (OUN) ] Towards a software architecture for reusable game components
	\item [08 Ali Mirsoleimani (UL) ] Structured Parallel Programming for Monte Carlo Tree Search
	\item [09 Myriam Traub (UU) ] Measuring Tool Bias and Improving Data Quality for Digital Humanities Research
	\item [10 Alifah Syamsiyah (TUE) ] In-database Preprocessing for Process Mining
	\item [11 Sepideh Mesbah (TUD) ] Semantic-Enhanced Training Data AugmentationMethods for Long-Tail Entity Recognition Models
	\item [12 Ward van Breda (VU) ] Predictive Modeling in E-Mental Health: Exploring Applicability in Personalised Depression Treatment
	\item [13 Marco Virgolin (CWI) ] Design and Application of Gene-pool Optimal Mixing Evolutionary Algorithms for Genetic Programming
	\item [14 Mark Raasveldt (CWI/UL) ] Integrating Analytics with Relational Databases
	\item [15 Konstantinos Georgiadis (OUN) ] Smart CAT: Machine Learning for Configurable Assessments in Serious Games
	\item [16 Ilona Wilmont (RUN) ] Cognitive Aspects of Conceptual Modelling
	\item [17 Daniele Di Mitri (OUN) ] The Multimodal Tutor: Adaptive Feedback from Multimodal Experiences
	\item [18 Georgios Methenitis (TUD) ] Agent Interactions \& Mechanisms in Markets with Uncertainties: Electricity Markets in Renewable Energy Systems
	\item [19 Guido van Capelleveen (UT) ] Industrial Symbiosis Recommender Systems
	\item [20 Albert Hankel (VU) ] Embedding Green ICT Maturity in Organisations

\end{description}
\end{multicols}

